A generalized stacked reinforcement learning method for sampled systems

A common setting of reinforcement learning (RL) is a Markov decision process (MDP) in which the environment is a stochastic discrete-time dynamical system. Whereas MDPs are suitable in such applications as video-games or puzzles, physical systems are time-continuous. A general variant of RL is of digital format, where updates of the value (or cost) and policy are performed at discrete moments in time. The agent-environment loop then amounts to a sampled system, whereby sample-and-hold is a specific case. In this paper, we propose and benchmark two RL methods suitable for sampled systems. Specifically, we hybridize model-predictive control (MPC) with critics learning the optimal Q- and value (or cost-to-go) function. Optimality is analyzed and performance comparison is done in an experimental case study with a mobile robot.

==> preamble-AIDA.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% AIDA %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{xspace}
\usepackage{soul}
\usepackage{mathtools}
\usepackage{makecell}
%\usepackage{cite}
\usepackage{todonotes}
\usepackage{nicefrac}

%%%% Arrow notation
\newcommand{\ra}{\rightarrow}
\newcommand{\rra}{\rightrightarrows}
\newcommand{\la}{\leftarrow}

%%%% Abbreviations
\newcommand{\ie}{\unskip, i.\,e.,\xspace}
\newcommand{\eg}{\unskip, e.\,g.,\xspace}
\newcommand{\pd}{p.\,d.\xspace}
\newcommand{\sut}{\text{s.\,t.\,}}
\newcommand{\rt}{r.\,t.\xspace}

%%%% Wraps
\newcommand{\nrm}[1]{\left\lVert#1\right\rVert}
\newcommand{\diag}[1]{\ensuremath{\text{diag}}\left(#1\right)}
\newcommand{\abs}[1]{\left\lvert#1\right\rvert}
\newcommand{\scal}[1]{\left\langle#1\right\rangle}
\newcommand{\tr}[1]{\ensuremath{\text{tr}}\left(#1\right)}
\newcommand{\E}[1]{\mathbb E\left[#1\right]}
\newcommand{\PP}[1]{\mathbb P\left[#1\right]}

%%%% Set notation
\newcommand{\N}{\ensuremath{\mathbb{N}}}
\newcommand{\Z}{\ensuremath{\mathbb{Z}}}
\newcommand{\Q}{\ensuremath{\mathbb{Q}}}
\newcommand{\R}{\ensuremath{\mathbb{R}}}

\newcommand{\С}{\ensuremath{\mathbb{С}}}
%\renewcommand{\C}{\ensuremath{\mathbb{C}}}  % In case of error with the \C command

\newcommand{\T}{\ensuremath{\mathbb{T}}}
\newcommand{\X}{\ensuremath{\mathbb{X}}}
\newcommand{\Y}{\ensuremath{\mathbb{Y}}}
\newcommand{\F}{\ensuremath{\mathbb{F}}}

\newcommand{\U}{\ensuremath{\mathbb{U}}}
%\renewcommand{\U}{\ensuremath{\mathbb{U}}}  % In case of error with the \U command

\newcommand{\sm}{\ensuremath{\setminus}}
\newcommand{\set}[1]{\ensuremath{\mathbb{#1}}}

\let\oldemptyset\emptyset
\let\emptyset\varnothing

%%%% Miscellaneous commands
\newcommand*\diff{\mathop{}\!\mathrm{d}}
\newcommand{\eps}{\ensuremath{\varepsilon}}
\newcommand{\sgn}{\ensuremath{\text{sgn}}}
\newcommand{\spc}{\ensuremath{\,\,}}
\newcommand{\diam}{\ensuremath{\text{diam}}}
\newcommand{\dom}{\ensuremath{\text{dom}}}
\newcommand{\ramp}{\ensuremath{\text{ramp}}}
\newcommand{\pdiff}[2]{ \ensuremath{ \frac{\partial {#1}}{\partial {#2}} } }

\newcommand{\ball}{\ensuremath{\mathcal B}}
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{\node[shape=circle,draw,inner sep=1pt] (char) {#1};}}

\newcommand{\co}{\ensuremath{\overline{\text{co}}}}

\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}

%%%% Review
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\definecolor{dgreen}{rgb}{0.0, 0.5, 0.0}
\newcommand{\green}[1]{\textcolor{dgreen}{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
